Lepton universality tests and searches for new physics in charged current decays at Belle II

We present recent tests of lepton universality as crucial probes of the Standard Model in semileptonic $B$-meson decays at Belle II. All presented analyses use a data sample collected at the $\Upsilon(4S)$ resonance by the Belle II experiment corresponding to an integrated luminosity of $189\,\mathrm{fb}^{-1}$. We report three analyses that probe light-lepton universality: The first measurement of a complete set of five angular asymmetries using $\bar{B}^0 \to D^{*+} \ell^- \bar{\nu}_\ell$ decays, followed by a measurement of the forward-backward asymmetry in untagged $\bar{B}^0 \to D^{*+} \ell^- \bar{\nu}_\ell$ decays, and finally, measurements of the branching-fraction ratios $R(D^{*+}_{e/\mu}) = \mathcal{B}(\bar{B}^0 \to D^{*+} e^- \bar{\nu}_e) / \mathcal{B}(\bar{B}^0 \to D^{*+} \mu^- \bar{\nu}_\mu)$, using the same untagged data set, along with the first measurement of the inclusive light-lepton ratio $R(X_{e/\mu}) = \mathcal{B}(\bar{B} \to X e^- \bar{\nu}_e) / \mathcal{B}(\bar{B} \to X \mu^- \bar{\nu}_\mu)$. Furthermore, we present two tests of heavy-to-light lepton universality. In the first test, we report the measurement of the branching-fraction ratio $R(D^{*}_{\tau/\ell})$ using hadronic tagging. In the second test, we present the first measurement of the inclusive ratio $R(X_{\tau/\ell})$. All presented results are consistent with their corresponding Standard Model predictions and, where applicable, with the experimental world averages.

==> 00_definitions.tex <==

\RequirePackage{xspace}

% A few useful definitions.
%\newcommand{\mysim}{\sim\!}
%\newcommand{\mysimeq}{\simeq\!}

%\newcommand{\pho}{\phantom{0}}
%\newcommand{\phplus}{\phantom{+}}

% general
%\newcommand*{\invfb}{\ensuremath{\mbox{\,fb}^{-1}}\xspace}

% SM Properties
\newcommand*{\lagrange}{\ensuremath{\mathcal{L}}\xspace}
\newcommand*{\aem}{\ensuremath{\alpha_\text{em}}\xspace}
\newcommand*{\aw}{\ensuremath{\alpha_\text{w}}\xspace}
\newcommand*{\as}{\ensuremath{\alpha_\text{s}}\xspace}
\newcommand*{\gw}{\ensuremath{g_\text{w}}\xspace}
\newcommand*{\gs}{\ensuremath{g_\text{s}}\xspace}
\newcommand*{\gfermi}{\ensuremath{G_\text{F}}\xspace}

\newcommand*{\uone}{\ensuremath{\text{U(1)}_\text{Y}}\xspace}
\newcommand*{\uoneem}{\ensuremath{\text{U(1)}_\text{em}}\xspace}
\newcommand*{\sutwo}{\ensuremath{\text{SU(2)}_\text{L}}\xspace}
\newcommand*{\suthree}{\ensuremath{\text{SU(3)}_\text{C}}\xspace}
\newcommand*{\sun}{\ensuremath{\text{SU(N)}}\xspace}

\newcommand*{\higgspot}{\ensuremath{V_\text{Higgs}(\Phi)}\xspace}

\newcommand*{\vckm}{\ensuremath{V_\text{CKM}}\xspace}
\newcommand*{\lqcd}{\ensuremath{\Lambda_\text{QCD}}\xspace}

%Allgemeines

%\newcommand*{\fb}{\femto\barn}

% Kinematics
%\newcommand*{\met}{\ensuremath{E_\text{T}^\text{miss}}\xspace}
%\newcommand*{\pt}{\ensuremath{p_\text{T}}\xspace}
%\newcommand*{\abseta}{\ensuremath{|\eta|}\xspace}
% multiplicities
%\newcommand*{\ntau}{\ensuremath{N_\tau}\xspace}
%\newcommand*{\nele}{\ensuremath{N_e}\xspace}
%\newcommand*{\nmu}{\ensuremath{N_\mu}\xspace}
%\newcommand*{\nlep}{\ensuremath{N_\text{lep}}\xspace}
%\newcommand*{\njet}{\ensuremath{N_\text{jets}}\xspace}
%\newcommand*{\njetfourty}{\ensuremath{N_\text{jets, 40 GeV}}\xspace}
%\newcommand*{\nbjet}{\ensuremath{N_{\bqu-\text{jets}}}\xspace}
%\newcommand*{\nobjects}{\ensuremath{N_\text{objects}}\xspace}
%\newcommand*{\ntauvertex}{\ensuremath{N_\tau^\text{vertex}}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   BELLE II SPECIFIC   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%% COLLABORATION NAMES %%%%
% B factories
\def\belletwo {Belle~II\xspace}
\def\belle{Belle\xspace}
\def\babar{\textsc{\textit{BaBar}}\xspace}
\def\cleo{CLEO\xspace}
\def\argus{ARGUS\xspace}
% CERN, LHC, LEP etc
\def\cern{CERN\xspace}
\def\lhc{LHC\xspace}
\def\atlas{ATLAS\xspace}
% \def\CMS{CMS\xspace} % already used as command for center-of-mass system...
\def\lhcb{LHCb\xspace}

\def\lep{LEP\xspace}
\def\aleph{ALEPH\xspace}
\def\opal{OPAL\xspace}
\def\lthree{L3\xspace}
\def\delphi{DELPHI\xspace}
% MC generator stuff, software packages etc
\def\minuit{\textsc{\footnotesize{MINUIT}}\xspace}
\def\hesse{\textsc{\footnotesize{HESSE}}\xspace}
\def\minos{\textsc{\footnotesize{MINOS}}\xspace}
\def\genfit{\textsc{\small{Genfit2}}\xspace}
\def\evtgen{\textsc{\small{EvtGen}}\xspace}
\def\kkmc{\textsc{\footnotesize{KKMC}}\xspace}
\def\pythia{\textsc{\footnotesize{PYTHIA}}\xspace}
\def\photos{\textsc{\small{Photos}}\xspace}
\def\geant{\textsc{\small{Geant4}}\xspace}
\def\basftwo{{\fontfamily{qcr}\selectfont basf2}\xspace}
\def\cpp{\textsc{\small{C++}}\xspace}
\def\python{\textsc{\small{Python}}\xspace}
\def\hammer{\textsc{\footnotesize{HAMMER}}\xspace}

\def\mcof{MC14\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\y     {\ensuremath{\gamma}\xspace}
%\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
%\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}
%
%\def\ega    {\ensuremath{e\gamma}\xspace}
%\def\game   {\ensuremath{\gamma e^-}\xspace}
%\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}
\def\g      {\ensuremath{g}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}
\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\ele   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace}
%\def\epem       {\ensuremath{e^+e^-}\xspace}
%\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
%\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}

\def\mtau       {\ensuremath{\tau}\xspace}
\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
%\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
%\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
%\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
%% \num conflicts with siunitx
\def\numu        {\ensuremath{\nu_\mu}\xspace}
\def\numub       {\ensuremath{\nub_\mu}\xspace}
%\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
%\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
%\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace}
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace}
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\D       {\ensuremath{D}\xspace}
%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dst   {\ensuremath{D^*}\xspace}
\def\Dstb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstz  {\ensuremath{D^{*0}}\xspace}
\def\Dstzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstp  {\ensuremath{D^{*+}}\xspace}
\def\Dstm  {\ensuremath{D^{*-}}\xspace}
\def\Dstpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstmp {\ensuremath{D^{*\mp}}\xspace}
\def\DorDst   {\ensuremath{D^{(*)}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}
\def\DsorDsst   {\ensuremath{D_s^{(*)}}\xspace}
\def\Dstst {\ensuremath{D^{**}}\xspace}
\def\Dzstar  {\ensuremath{D_{0}^{*}}\xspace}
\def\Done  {\ensuremath{D_{1}}\xspace}
\def\Doneprime  {\ensuremath{D'_{1}}\xspace}
\def\Dtwostar  {\ensuremath{D_{2}^{*}}\xspace}
\def\DDstorDstst   {\ensuremath{D^{(*, **)}}\xspace}

\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace}
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}
\def\SixS  {\Y6S}

\def\chic#1{\ensuremath{\chi_{c#1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\pbar  {\kern 0.12em\overline{\kern -0.12em p}{}\xspace}
%\def\antiproton {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\nbar  {\kern 0.06em\overline{\kern -0.06em n}{}\xspace}
%\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\gevsqcccc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V^2\!/}c^4}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

%\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}

\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}
\def\sy    {\ensuremath{\sigma_y}\xspace}
\def\sz    {\ensuremath{\sigma_z}\xspace}


\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
		\lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
		\lower.35em\hbox{$\sim$}~}\xspace}

%%%%%%%%%%%%%%%%
%% R(X) analysis
%%%%%%%%%%%%%%%%

% general 
%\newcommand*{\cms}{\ensuremath{\text{c.m.}}\xspace}
\newcommand*{\cms}{\ensuremath{{*}}\xspace}
\newcommand*{\cmstext}{c.~m.\xspace}
\newcommand*{\Ecms}{\ensuremath{E^\cms}\xspace} % I should always use sqrt(s) instead of E(CMS)?!
\newcommand*{\sqrts}{\ensuremath{\sqrt{s}}\xspace}
\newcommand*{\pcms}{\ensuremath{p^\cms}\xspace}
\newcommand*{\lumi}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\lumion}{\ensuremath{\SI{189}{\per\femto\barn}}\xspace}
\newcommand{\lumioff}{\ensuremath{\SI{18}{\per\femto\barn}}\xspace}

%detector stuff
\newcommand{\cherenkovangle}{\ensuremath{\theta_\text{C}}\xspace}

% important quantities
% signal extraction:
\newcommand*{\mmsq}{\ensuremath{M_\mathrm{miss}^2}\xspace}
\newcommand*{\mx}{\ensuremath{M_X}\xspace}
\newcommand*{\qsq}{\ensuremath{q^2}\xspace}

% lepton momenta:
\newcommand{\plB}{\ensuremath{p_{\ell}^{B}}\xspace}
\newcommand{\peB}{\ensuremath{p_{e}^{B}}\xspace}
\newcommand{\pmuB}{\ensuremath{p_{\mu}^{B}}\xspace}
%\newcommand*{\plrf}{\ensuremath{p_\ell^B}\xspace}
%\newcommand*{\perf}{\ensuremath{p_e^B}\xspace}
%\newcommand*{\pmurf}{\ensuremath{p_\mu^B}\xspace}
\newcommand*{\pllab}{\ensuremath{p_{\ell}}\xspace}
\newcommand*{\plcms}{\ensuremath{p_\ell^\cms}\xspace}
\newcommand*{\pelab}{\ensuremath{p_{e}}\xspace}
\newcommand*{\pmulab}{\ensuremath{p_{\mu}}\xspace}
\newcommand*{\pT}{\ensuremath{p_{\text{T}}}\xspace}
\newcommand*{\plT}{\ensuremath{p_{\ell \text{T}}}\xspace}
\newcommand*{\peT}{\ensuremath{p_{e \text{T}}}\xspace}
\newcommand*{\pmuT}{\ensuremath{p_{\mu \text{T}}}\xspace}
\newcommand*{\thetallab}{\ensuremath{\theta_{\ell}}\xspace}


% tag-side / sig-side quantities
\newcommand*{\btag}{\ensuremath{B_\text{tag}}\xspace}
\newcommand*{\bsig}{\ensuremath{B_\text{sig}}\xspace}
\newcommand{\mbsig}{\ensuremath{M_{\bsig}}\xspace}
\newcommand*{\feiprob}{\ensuremath{\mathcal{P}_\text{FEI}}\xspace}
\newcommand*{\eeclfei}{\ensuremath{E_\text{ECL}}\xspace}
\newcommand*{\ecmsfei}{\ensuremath{E_\text{tot.}^\cms}\xspace}
\newcommand{\mbc}{\ensuremath{M_{\textrm{bc}}}\xspace}
\newcommand*{\mbccorr}{\ensuremath{M_\text{bc}^\text{corr}}\xspace}
\newcommand{\deltaE}{\ensuremath{\Delta E}\xspace}
\newcommand*{\deltaEcorr}{\ensuremath{\Delta E^\text{corr}}\xspace}

\newcommand*{\totscaleoffres}{\ensuremath{c_\text{off-res}}\xspace}
\newcommand*{\escaleoffres}{\ensuremath{c_\text{off-res}^E}\xspace}
\newcommand*{\ecmsoffres}{\ensuremath{\sqrt{s}_\text{off-res}}\xspace}
\newcommand*{\ecmsonres}{\ensuremath{\sqrt{s}_{\FourS}}\xspace}


% R ratios and branching fractions.
\newcommand{\RX}{\ensuremath{R(X_{\tau/\ell})}\xspace}
\newcommand{\RXe}{\ensuremath{R(X_{\tau/e})}\xspace}
\newcommand{\RXmu}{\ensuremath{R(X_{\tau/\mu})}\xspace}
\newcommand{\Remu}{\ensuremath{R(X_{e/\mu})}\xspace}
\newcommand{\Remufid}{\ensuremath{R(X_{e/\mu}\mid \plB > \SI{1.3}{\GeV})}\xspace}
\newcommand{\RDstemu}{\ensuremath{R(\Dstp_{e/\mu})}\xspace}
\newcommand{\RXc}{\ensuremath{R(X_c)}\xspace}
\newcommand{\RXu}{\ensuremath{R(X_u)}\xspace}
\newcommand{\RD}{\ensuremath{R(D_{\tau/\ell})}\xspace}
\newcommand{\RDst}{\ensuremath{R(D^{*}_{\tau/\ell})}\xspace}
\newcommand{\RDorDst}{\ensuremath{R(\DorDst_{\tau/\ell})}\xspace}
\newcommand{\RDstst}{\ensuremath{R(D^{**})}\xspace}
\newcommand{\RDDstorDstst}{\ensuremath{R(\DDstorDstst)}\xspace}
% R()X_e/mu) related
\newcommand*{\Nemu}{\ensuremath{N_{e/ \mu}}\xspace}
\newcommand*{\Epsemu}{\ensuremath{\epsilon_{e/ \mu}}\xspace}
\newcommand*{\Rmue}{\ensuremath{\mathcal{R}(X_{\mu / e})}\xspace}
\newcommand*{\Nmue}{\ensuremath{N_{\mu / e}}\xspace}
\newcommand*{\Epsmue}{\ensuremath{\epsilon_{\mu / e}}\xspace}
\newcommand*{\RemuXtau}{\ensuremath{\mathcal{R}(X_{e/\mu}^{\,\tau \to})}\xspace}

% Event types
\newcommand*{\gap}{\ensuremath{D_\text{gap}^{**}}\xspace}

% tau -> ... nu
\newcommand{\taupinu}{\ensuremath{\tau \to \pi \nu}\xspace}
\newcommand{\taurhonu}{\ensuremath{\tau \to \rho \nu}\xspace}
\newcommand{\taulnunu}{\ensuremath{\tau \to \ell \nu \nu}\xspace}
\newcommand{\tauenunu}{\ensuremath{\tau^- \to e^- \nueb \nut}\xspace}
\newcommand{\taumununu}{\ensuremath{\tau^- \to \mu^- \numub \nut}\xspace}

% X ell/tau nu:
\newcommand{\xtaunu}{\ensuremath{X \tau^- \nutb}\xspace}
\newcommand{\xtautolnu}{\ensuremath{X [\taulnunu] \nutb}\xspace}
\newcommand{\xtautoenu}{\ensuremath{X [\tauenunu] \nutb}\xspace}
\newcommand{\xtautomunu}{\ensuremath{X [\taumununu] \nutb}\xspace}
%\newcommand{\xtaulnu}{\ensuremath{X \tau(\ell) \nu}\xspace}
\newcommand{\xctaunu}{\ensuremath{X_c \tau^- \nutb}\xspace}
%\newcommand{\xctaulnu}{\ensuremath{X_c \tau(\ell) \nu}\xspace}
\newcommand{\xutaunu}{\ensuremath{X_u \tau^- \nutb}\xspace}
%\newcommand{\xcutaulnu}{\ensuremath{X_{c, (u)} \tau(\ell) \nu}\xspace}
\newcommand{\xlnu}{\ensuremath{X \ell^- \nulb}\xspace}
\newcommand{\xenu}{\ensuremath{X e^- \nueb}\xspace}
\newcommand{\xmunu}{\ensuremath{X \mu^- \numub}\xspace}
\newcommand{\xclnu}{\ensuremath{X_c \ell^- \nulb}\xspace}
\newcommand{\xcenu}{\ensuremath{X_c e^- \nueb}\xspace}
\newcommand{\xulnu}{\ensuremath{X_u \ell^- \nulb}\xspace}

\newcommand*{\dtaunu}{\ensuremath{D  \tau^-  \nutb}\xspace}
\newcommand*{\dsttaunu}{\ensuremath{D^{*}  \tau^-  \nutb}\xspace}
\newcommand*{\dordsttaunu}{\ensuremath{\DorDst \tau^-  \nutb}\xspace}
\newcommand*{\dststtaunu}{\ensuremath{D^{**}  \tau^- \nutb}\xspace}
\newcommand*{\dordstsktaunu}{\ensuremath{\DsorDsst K \tau \nutb}\xspace}
\newcommand*{\dordstpipitaunu}{\ensuremath{\DorDst \pi \pi \tau^- \nutb}\xspace}
\newcommand*{\dordstetataunu}{\ensuremath{\DorDst \eta \tau^- \nutb}\xspace}
\newcommand*{\gaptaunu}{\ensuremath{\gap \tau^- \nutb}\xspace}
\newcommand*{\xstautau}{\ensuremath{X_s \tau \tau}\xspace}

\newcommand*{\dlnu}{\ensuremath{D \ell^- \nulb}\xspace}
\newcommand*{\dstlnu}{\ensuremath{D^{*} \ell^- \nulb}\xspace}
\newcommand*{\dstenu}{\ensuremath{D^{*} e^- \nueb}\xspace}
\newcommand*{\dstmunu}{\ensuremath{D^{*} \mu^- \numub}\xspace}
\newcommand*{\dordstlnu}{\ensuremath{\DorDst  \ell^-  \nulb}\xspace}
\newcommand*{\ddstordststlnu}{\ensuremath{\DDstorDstst  \ell^-  \nulb}\xspace}
\newcommand*{\dststlnu}{\ensuremath{D^{**}  \ell^-  \nulb}\xspace}
\newcommand*{\dordstsklnu}{\ensuremath{\DsorDsst  K  \ell^-  \nulb}\xspace}
\newcommand*{\dordstpilnu}{\ensuremath{\DorDst  \pi  \ell^-  \nulb}\xspace}
\newcommand*{\dordstpipilnu}{\ensuremath{\DorDst  \pi  \pi  \ell^-  \nulb}\xspace}
\newcommand*{\dordstetalnu}{\ensuremath{\DorDst  \eta  \ell^-  \nulb}\xspace}
\newcommand*{\gaplnu}{\ensuremath{\gap  \ell  \nulb}\xspace}
\newcommand*{\xsll}{\ensuremath{X_s \ell  \ell}\xspace}

% B -> event types
\newcommand{\bxtaulnu}{\ensuremath{\Bb \to \xtaulnu}\xspace}
\newcommand{\bxtaunu}{\ensuremath{\Bb \to \xtaunu}\xspace}
\newcommand{\bxctaunu}{\ensuremath{\Bb \to \xctaunu}\xspace}
\newcommand{\bxutaunu}{\ensuremath{\Bb \to \xutaunu}\xspace}
\newcommand{\bxtautolnu}{\ensuremath{\Bb \to \xtautolnu}\xspace}
\newcommand{\bxtautoenu}{\ensuremath{\Bb \to \xtautoenu}\xspace}
\newcommand{\bxtautomunu}{\ensuremath{\Bb \to \xtautomunu}\xspace}
\newcommand{\bxlnu}{\ensuremath{\Bb \to \xlnu}\xspace}
\newcommand{\bxclnu}{\ensuremath{\Bb \to \xclnu}\xspace}
\newcommand{\bxulnu}{\ensuremath{\Bb \to \xulnu}\xspace}
\newcommand{\bxenu}{\ensuremath{\Bb \to \xenu}\xspace}
\newcommand{\bxmunu}{\ensuremath{\Bb \to \xmunu}\xspace}

\newcommand{\bquxtaunu}{\ensuremath{b\to \xtaunu}\xspace}
\newcommand{\bclnu}{\ensuremath{b \to c \ell \nu}\xspace}
\newcommand{\bulnu}{\ensuremath{b \to u \ell \nu}\xspace}
\newcommand{\bctaunu}{\ensuremath{b \to c \tau \nu}\xspace}
%\newcommand{\bctaulnu}{\ensuremath{b \to c \tau(\ell) \nu}\xspace}
%\newcommand{\butaulnu}{\ensuremath{b \to u \tau(\ell) \nu}\xspace}
% D, D* modes
%\newcommand{\bdtaulnu}{\ensuremath{B \to \dtaulnu}\xspace}
\newcommand{\bdtaunu}{\ensuremath{\Bb \to \dtaunu}\xspace}
\newcommand{\bdlnu}{\ensuremath{\Bb \to \dlnu}\xspace}
%\newcommand{\bdsttaulnu}{\ensuremath{B \to \dsttaulnu}\xspace}
\newcommand{\bdsttaunu}{\ensuremath{\Bb \to \dsttaunu}\xspace}
\newcommand{\bdstlnu}{\ensuremath{\Bb \to \dstlnu}\xspace}
\newcommand{\bdstenu}{\ensuremath{\Bb \to \dstenu}\xspace}
\newcommand{\bdstmunu}{\ensuremath{\Bb \to \dstmunu}\xspace}
\newcommand{\bdordsttaulnu}{\ensuremath{\Bb \to \dordsttaulnu}\xspace}
\newcommand{\bdordsttaunu}{\ensuremath{\Bb \to \dordsttaunu}\xspace}
\newcommand{\bdordstlnu}{\ensuremath{\Bb \to \dordstlnu}\xspace}
\newcommand{\bddstordststnu}{\ensuremath{\Bb \to \ddstordststlnu}\xspace}
% D** modes and gap modes
\newcommand{\bdststtaunu}{\ensuremath{\Bb \to \dststtaunu}\xspace}
\newcommand{\bdststlnu}{\ensuremath{\Bb \to \dststlnu}\xspace}
\newcommand{\bdordstpipitaunu}{\ensuremath{\Bb \to \dordstpipitaunu}\xspace}
\newcommand{\bdordstetataunu}{\ensuremath{\Bb \to \dordstetataunu}\xspace}
\newcommand{\bdordstpilnu}{\ensuremath{\Bb \to \dordstpilnu}\xspace}
\newcommand{\bdordstpipilnu}{\ensuremath{\Bb \to \dordstpipilnu}\xspace}
\newcommand{\bdordstetalnu}{\ensuremath{\Bb \to \dordstetalnu}\xspace}
\newcommand{\bgaplnu}{\ensuremath{\Bb \to \gaplnu}\xspace}
% charge specific:
\newcommand*{\dordstpippimlnu}{\ensuremath{\DorDst  \pi^+  \pi^-  \ell  \nu}\xspace}
\newcommand{\bzdstmlpnu}{\ensuremath{B^{0} \to D^{*-} \ell^{+} \nu}\xspace}
\newcommand{\bzdstmepnu}{\ensuremath{B^{0} \to D^{*-} e^{+} \nu}\xspace}
\newcommand{\bzdstmmupnu}{\ensuremath{B^{0} \to D^{*-} \mu^{+} \nu}\xspace}
% BFs
\newcommand{\BF}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\BFxtaunu}{\ensuremath{\mathcal{B}(\bxtaunu)}\xspace}
\newcommand{\BFdtaunu}{\ensuremath{\mathcal{B}(\bdtaunu)}\xspace}
\newcommand{\BFdsttaunu}{\ensuremath{\mathcal{B}(\bdsttaunu)}\xspace}
\newcommand{\BFdordsttaunu}{\ensuremath{\mathcal{B}(\bdordsttaunu)}\xspace}
\newcommand{\BFdgapxutaunu}{\ensuremath{\mathcal{B}(B \to D^{**}_\text{(gap)}/X_u \tau \nu)}\xspace}
\newcommand{\BFxlnu}{\ensuremath{\mathcal{B}(\bxlnu)}\xspace}
\newcommand{\BFxenu}{\ensuremath{\mathcal{B}(\bxenu)}\xspace}
\newcommand{\BFxmunu}{\ensuremath{\mathcal{B}(\bxmunu)}\xspace}
\newcommand{\BFxclnu}{\ensuremath{\mathcal{B}(\bxclnu)}\xspace}
\newcommand{\BFxulnu}{\ensuremath{\mathcal{B}(\bxulnu)}\xspace}
\newcommand{\BFdlnu}{\ensuremath{\mathcal{B}(\bdlnu)}\xspace}
\newcommand{\BFdstlnu}{\ensuremath{\mathcal{B}(\bdstlnu)}\xspace}
\newcommand{\BFdstenu}{\ensuremath{\mathcal{B}(\bdstenu)}\xspace}
\newcommand{\BFdstmunu}{\ensuremath{\mathcal{B}(\bdstmunu)}\xspace}
\newcommand{\BFdordstlnu}{\ensuremath{\mathcal{B}(\bdordstlnu)}\xspace}
\newcommand{\BFdgapxulnu}{\ensuremath{\mathcal{B}(B \to D^{**}_\text{(gap)}/X_u \ell \nu)}\xspace}
% LEP:
\newcommand{\BFLEPxtaunu}{\ensuremath{\mathcal{B}($b$\text{-admix} \to X \tau \nu)}\xspace}
% Misc. decays, LHCb etc:
\newcommand{\BFdtautohadnu}{\ensuremath{\mathcal{B}(B^0 \to D^{*-} [\tau^+ \to \pi^+ \pi^- \pi^+ (\pi^0) \nutb] \nut)}\xspace}
\newcommand{\BFdstpipipi}{\ensuremath{\mathcal{B}(B^0 \to D^{*-} \pi^+ \pi^- \pi^+)}\xspace}
\newcommand{\BFkpee}{\ensuremath{\mathcal{B}(\Bp \to K^+ e^+ e^-)}\xspace}
\newcommand{\BFkpmumu}{\ensuremath{\mathcal{B}(\Bp \to K^+ \mu^+ \mu^-)}\xspace}
\newcommand{\BFksee}{\ensuremath{\mathcal{B}(\Bz \to \KS e^+ e^-)}\xspace}
\newcommand{\BFksmumu}{\ensuremath{\mathcal{B}(\Bz \to \KS \mu^+ \mu^-)}\xspace}
\newcommand{\bpknunu}{\ensuremath{\Bp \to K^{+} \nu\nub}\xspace}
% tau -> ell nu nu:
\newcommand{\BFtaulnunu}{\ensuremath{\mathcal{B}(\taulnunu)}\xspace}


% Likelihood fit
% command \llh is already defined when I talk about PID.
\newcommand*{\Nmeas}{\ensuremath{N^\text{meas}}\xspace}
\newcommand*{\Nsel}{\ensuremath{N^\text{sel}}\xspace}
\newcommand*{\Ngen}{\ensuremath{N^\text{gen}}\xspace}
